On the Convergence of Inexact Predictor-Corrector Methods for Linear Programming

Interior point methods (IPMs) are a common approach for solving linear programs (LPs) with strong theoretical guarantees and solid empirical performance. The time complexity of these methods is dominated by the cost of solving a linear system of equations at each iteration. In common applications of linear programming, particularly in machine learning and scientific computing, the size of this linear system can become prohibitively large, requiring the use of iterative solvers, which provide an approximate solution to the linear system. However, approximately solving the linear system at each iteration of an IPM invalidates the theoretical guarantees of common IPM analyses. To remedy this, we theoretically and empirically analyze (slightly modified) predictor-corrector IPMs when using approximate linear solvers: our approach guarantees that, when certain conditions are satisfied, the number of IPM iterations does not increase and that the final solution remains feasible. We also provide practical instantiations of approximate linear solvers that satisfy these conditions for special classes of constraint matrices using randomized linear algebra.

==> Definitions.tex <==
% 2014 written by S V N Vishwanathan (vishy@ucsc.edu)
% 2015 modified by Jiasen Yang (jiaseny@purdue.edu)

\RequirePackage{latexsym}
\RequirePackage{amsmath}
% \RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage[mathscr]{euscript}

%%% Macros for this paper

\newcommand{\tolSolve}{\delta_{\epsilon, n}}
\newcommand{\tolSolveNoN}{\delta_{\epsilon}}

\newcommand{\xtilde}{\Tilde{\xb}}
\newcommand{\stilde}{\Tilde{\sbb}}
\newcommand{\ytilde}{\Tilde{\yb}}
\newcommand{\mutilde}{\Tilde{\mu}}
\newcommand{\ztilde}{\Tilde{\zb}}
\newcommand{\Ocaltil}{\widetilde{\mathcal{O}}}

\newcommand{\dxtilde}{\Delta \Tilde{\xb}}
\newcommand{\dstilde}{\Delta \Tilde{\sbb}}
\newcommand{\dytilde}{\Delta \Tilde{\yb}}

\newcommand{\dxexact}{\Delta \xb}
\newcommand{\dsexact}{\Delta \sbb}
\newcommand{\dyexact}{\Delta \yb}

\newcommand{\kfinal}{{k^*}}
\newcommand{\xopt}{\xb^*}
\newcommand{\yopt}{\yb^*}
\newcommand{\sopt}{\sbb^*}
\newcommand{\muopt}{\mu^*}

%%%%   Setting these to have no tilde....same as xopt, etc.
\newcommand{\mutopt}{\mu^*}
\newcommand{\xtopt}{\xb^*}
\newcommand{\ytopt}{\yb^*}
\newcommand{\stopt}{\sbb^*}

\newcommand{\solve}{\texttt{Solve}}
\newcommand{\solvev}{\texttt{Solve}^{\vb}}

%%%%%%

\newcommand{\D}{\text{d}}
\newcommand{\ex}{\mathbb{E}}
\newcommand{\Ex}[1]{\mbox{}\mathbb{E}\left[#1\right]}
\newcommand{\Var}[1]{\mbox{}\textup{Var}\left(#1\right)}
\newcommand{\Cov}[1]{\mbox{}\textup{Cov}\left(#1\right)}
\newcommand{\Tr}[1]{\mbox{}\textup{tr}\left(#1\right)}
\newcommand{\Trsq}[1]{\mbox{}\textup{tr}^2\left(#1\right)}
% \newcommand{\pr}{\mathbb{P}}
\newcommand{\pr}[1]{\mbox{}\mathbb{P}\left(#1\right)}
\newcommand{\kl}[2]{\mbox{}\mathbb{KL}\left(#1\,||\,#2\right)}
\newcommand{\tAb}{\widetilde{\Ab}}
\newcommand{\tp}{\widetilde{p}}
\newcommand{\ts}{\mathsf{T}}
% \newcommand{\ts}{\top}
% \newcommand{\ind}[1]{\mathbb{I}\{#1\}}
\newcommand{\ind}[1]{\mathds{1}\{#1\}}
\newcommand{\nnz}[1]{\mathsf{nnz}(#1)}
\newcommand{\Diag}[1]{\diag \left\{#1\right\}} % pseudoinverse
\newcommand{\Pinv}[1]{\mbox{}\left(#1\right)^{\dagger}} % pseudoinverse
\newcommand{\inv}[1]{\mbox{}\left(#1\right)^{-1}} % pseudoinverse
\newcommand{\RR}[2]{\mathbb{R}^{#1 \times #2}} % Real numbers
\newcommand{\R}{\mathbb{R}} % Real numbers
\newcommand{\Sqrt}[1]{#1^{\nicefrac{1}{2}}} % pseudoinverse
\newcommand{\defeq}{\triangleq}
% \newcommand{\var}{\text{var}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\disteq}{\stackrel{d}{=}}
\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\todo}[1]{\textcolor{red}{\texttt{TODO}: \emph{#1}}}


%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cbb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

% \newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Abtil}{\widetilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Ascr}{\mathscr{A}}
\newcommand{\Bscr}{\mathscr{B}}
\newcommand{\Cscr}{\mathscr{C}}
\newcommand{\Dscr}{\mathscr{D}}
\newcommand{\Escr}{\mathscr{E}}
\newcommand{\Fscr}{\mathscr{F}}
\newcommand{\Gscr}{\mathscr{G}}
\newcommand{\Hscr}{\mathscr{H}}
\newcommand{\Iscr}{\mathscr{I}}
\newcommand{\Jscr}{\mathscr{J}}
\newcommand{\Kscr}{\mathscr{K}}
\newcommand{\Lscr}{\mathscr{L}}
\newcommand{\Mscr}{\mathscr{M}}
\newcommand{\Nscr}{\mathscr{N}}
\newcommand{\Oscr}{\mathscr{O}}
\newcommand{\Pscr}{\mathscr{P}}
\newcommand{\Qscr}{\mathscr{Q}}
\newcommand{\Rscr}{\mathscr{R}}
\newcommand{\Sscr}{\mathscr{S}}
\newcommand{\Tscr}{\mathscr{T}}
\newcommand{\Uscr}{\mathscr{U}}
\newcommand{\Vscr}{\mathscr{V}}
\newcommand{\Wscr}{\mathscr{W}}
\newcommand{\Xscr}{\mathscr{X}}
\newcommand{\Yscr}{\mathscr{Y}}
\newcommand{\Zscr}{\mathscr{Z}}

\newcommand{\Ascrb}{\boldsymbol{\Ascr}}
\newcommand{\Bscrb}{\boldsymbol{\Bscr}}
\newcommand{\Cscrb}{\boldsymbol{\Cscr}}
\newcommand{\Dscrb}{\boldsymbol{\Dscr}}
\newcommand{\Escrb}{\boldsymbol{\Escr}}
\newcommand{\Fscrb}{\boldsymbol{\Fscr}}
\newcommand{\Gscrb}{\boldsymbol{\Gscr}}
\newcommand{\Hscrb}{\boldsymbol{\Hscr}}
\newcommand{\Iscrb}{\boldsymbol{\Iscr}}
\newcommand{\Jscrb}{\boldsymbol{\Jscr}}
\newcommand{\Kscrb}{\boldsymbol{\Kscr}}
\newcommand{\Lscrb}{\boldsymbol{\Lscr}}
\newcommand{\Mscrb}{\boldsymbol{\Mscr}}
\newcommand{\Nscrb}{\boldsymbol{\Nscr}}
\newcommand{\Oscrb}{\boldsymbol{\Oscr}}
\newcommand{\Pscrb}{\boldsymbol{\Pscr}}
\newcommand{\Qscrb}{\boldsymbol{\Qscr}}
\newcommand{\Rscrb}{\boldsymbol{\Rscr}}
\newcommand{\Sscrb}{\boldsymbol{\Sscr}}
\newcommand{\Tscrb}{\boldsymbol{\Tscr}}
\newcommand{\Uscrb}{\boldsymbol{\Uscr}}
\newcommand{\Vscrb}{\boldsymbol{\Vscr}}
\newcommand{\Wscrb}{\boldsymbol{\Wscr}}
\newcommand{\Xscrb}{\boldsymbol{\Xscr}}
\newcommand{\Xscrbh}{\hat{\Xscrb}}
\newcommand{\Yscrb}{\boldsymbol{\Yscr}}
\newcommand{\Zscrb}{\boldsymbol{\Zscr}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}
\newcommand{\Lmat}{\Lb}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}

\newcommand{\vol}{\text{vol}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}{Lemma}[section]
\fi

\ifx\proposition\undefined
\newtheorem{proposition}[lemma]{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}[theorem]{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}[theorem]{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
% \newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
% \newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{iid}}
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\cf}{\emph{cf.}\ }

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
% \newcommand{\ind}{\boldsymbol{\mathsf{I}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}
\newcommand{\Thetab}{\mathbf{\Theta}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}
\newcommand{\Lambdab}{\mathbf{\Lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}
\newcommand{\Omegab}{\boldsymbol{\Omega}}
\newcommand{\Phib}{\boldsymbol{\Phi}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ve}{\varepsilon}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


\newcommand{\Aone}{\textbf{A1}}
\newcommand{\Atwo}{\textbf{A2}}

\newcommand{\hWb}{\widehat{\Wb}}
% \newcommand{\Sreg}{\Sigmab_\mathsf{reg}}
\newcommand{\Sreg}{\widetilde{\Sigmab}}




==> pcu_2.tex <==

%%%  Predictor-Corrector Uncorrected
\section{Inexact Predictor-Corrector IPMs}
\label{section:pcu}

In this section, we analyze the \textit{inexact} predictor-corrector method (Algorithm~\ref{algo:pcu}) using an inexact linear solver $\solve$.  We follow the proof outline given in Section~\ref{section:overview} to prove the convergence guarantees and time complexity of Algorithm~\ref{algo:pcu}. As is common in predictor-corrector IPMs (see~\cite{wright1997primal}), we will assume that the matrix $\Ab$ has full row rank, ie., $rank(\Ab) = m \leq n$. See Section~\ref{section:low_rank} for extensions alleviating this constraint.

\begin{algorithm}[H] 
	\caption{Inexact Predictor-Corrector without correction} \label{algo:pcu}%
	\begin{algorithmic}
		
		\State \textbf{Input:}
		$\Ab\in\RR{\dimone}{\dimtwo}$, initial feasible point $(\xb^{0},\yb^{0},\sbb^{0}) \in \Ncal_2(0.25)$;  IPM tolerance $\epsilon> 0$, linear solver tolerance $\tolSolve > 0$. 
		
		\vspace{1mm}
		\State \textbf{Initialize:} ~$k\gets 0$;
		%------------------------------------------------------
		
		%%% Can choose tolerance adaptively at each step
		\vspace{1mm}
		\While{$\mu_k > 2\epsilon$} 

		\vspace{1mm}
		\textit{Predictor Step $(\sigma = 0)$:}
		\State(a) Compute $\dytilde = \texttt{Solve}(\Ab\Db^2\Ab^T, \Ab\xb, \tolSolve)$.
		%
		\vspace{1mm}
		%
		\State (b) Compute $\dxtilde$ and $\dstilde$ using eqn.~(\ref{eq:normal_uncorrected}).
		\vspace{1mm} 
		%
		\State (c) Set $\alpha = \min \left\{
        \nicefrac{1}{2},  ~
        \left( \nicefrac{\mu}{16(\|\dxtilde \circ \dstilde\|_2)} \right)^{1/2}
        \right\}$
		\vspace{1mm}
		%
		\State (d)~Compute $(\xb_k,\yb_k, \sbb_k) = (\xb_k,\yb_k,\sbb_k) + \alpha (\dxtilde_k,\dytilde_k,\dstilde_k)$. 
		\vspace{1mm}
		
		\textit{Corrector Step $(\alpha = 1, \sigma = 1)$:}
		\State(e) Compute $\dytilde = \texttt{Solve}(\Ab\Db^2\Ab^T, -\mu \Ab\Sb^{-1}\one_n + \Ab\xb, \tolSolve)$.
		%
		\vspace{1mm}
		%
		\State (f) Compute $\dxtilde$ and $\dstilde$ using eqn.~(\ref{eq:normal_uncorrected}).
		\vspace{1mm}
		%
		\State (g)~Compute $(\xb_{k+1},\yb_{k+1}, \sbb_{k+1}) = (\xb_k,\yb_k,\sbb_k) + (\dxtilde_k,\dytilde_k,\dstilde_k)$. 
		\vspace{1mm}
		
		
		\State (h) $k \gets k + 1$.
		
		\EndWhile
	\end{algorithmic}
\end{algorithm}

We will repeatedly express the inexact step as a function of the exact step. We start by expressing the difference of the steps computed by the \textit{exact} normal equations versus the \textit{inexact} normal equations, i.e. eqns.~(\ref{eq:normal_exact}) versus eqns.~(\ref{eq:normal_uncorrected}):
%
\begin{align}
    \dyexact - \dytilde &= (\Ab\Db^2\Ab^T)^{-1}\fb, \label{eq:ls_y_diff}\\
    \dsexact - \dstilde &= -\Ab^T(\dyexact - \dytilde)
    = -\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb, \label{eq:ls_s_diff}\\
    \dxexact - \dxtilde &= -\Db^2(\dsexact - \dstilde)
    = \Db^2\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb.  \label{eq:ls_x_diff}
\end{align}

We will prove that Algorithm~\ref{algo:pcu} converges to a point $(\xtopt, \ytopt, \stopt)$ satisfying $\mutopt < 2\epsilon$ and $\|\Ab\xtopt - \bb\|_2 < \epsilon$ in $\Ocal(\sqrt{n} \log \nicefrac{\mu_0}{\epsilon})$ outer iterations. First, we start with a technical result to bound $\|\dxtilde \circ \dstilde\|_2$.

\begin{lemma} \label{lemma:pcu_cross_bound}
    Let $(\xb,\yb,\sbb) \in \Ncal_2(\theta)$ and let $(\dxtilde, \dytilde, \dstilde)$ denote step calculated from the inexact normal equations (see eqn.~(\ref{eq:normal_uncorrected})). Then
    \begin{gather*}
        \|\dxtilde \circ \dstilde\|_2
        \leq \frac{\theta^2+n(1-\sigma)^2}{2^{3/2} (1-\theta)} \mu 
        + 2\sqrt{\frac{(\theta^2+n(1-\sigma)^2) \mu}{(1-\theta)}}  \|(\Ab\Db)^\dagger \fb\|_2
        + \|(\Ab\Db)^\dagger \fb\|_2^2.
    \end{gather*}
\end{lemma}

\begin{proof}
We start by expressing the inexact step as the difference from the corresponding exact step, using eqns.~(\ref{eq:ls_s_diff}) and~(\ref{eq:ls_x_diff}).  This will allow us to leverage results for exact predictor-corrector IPMs in our proof:
%
\begin{flalign*}
    \|\dxtilde \circ \dstilde\|_2 &= \|[\dxexact - (\dxexact - \dxtilde)] \circ [\dsexact - (\dsexact - \dstilde)] \|_2 \\
    %
    &\leq \|\dxexact \circ \dsexact\|_2 + \|\dxexact \circ (\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb) - \dsexact \circ (\Db^2\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb)\|_2  \\
    %
    &+ \|(\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb) \circ (\Db^2\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb)\|_2.
    %
\end{flalign*}

We will bound each of the three terms in the last inequality separately. Let $\Bcal_1 =  \|\dxexact \circ \dsexact\|_2$; 
$\Bcal_2 =  \|\dxexact \circ (\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb) - \dsexact \circ (\Db^2\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb)\|_2$; and 
\newline $\Bcal_3 =  \|(\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb) \circ (\Db^2\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb)\|_2$. Using eqn.~(\ref{eq:neighborhood_2}), we get a bound on $\Bcal_1$:
%
\begin{gather*}
    \Bcal_1 \leq \frac{\theta^2+n(1-\sigma)^2}{2^{3/2} (1-\theta)} \mu.
\end{gather*}

Next, we bound $\Bcal_2$.  First, we rearrange $\Bcal_2$ using properties of the Hadamard product (see Lemma \ref{lemma:hadamard_cauchy}) and Moore-Penrose pseudoinverse: 
\begin{flalign}
    \Bcal_2 &= \|\dxexact \circ (\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb) - \dsexact \circ (\Db^2\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb)\|_2 \nonumber\\
    &= \| [\Db^{-1}\dxexact] \circ [\Db\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb] - [\Db\dsexact] \circ [\Db\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb]\|_2 \nonumber\\
    %
    &= \|[\Db^{-1}\dxexact - \Db\dsexact] \circ [\Db\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb]\|_2 \nonumber\\
    %
    &\leq \|\Db^{-1}\dxexact - \Db\dsexact\|_2 \|(\Ab\Db)^\dagger \fb\|_2. 
    %
\end{flalign}

We now bound $\|\Db^{-1}\dxexact - \Db\dsexact\|_2$ by using the definitions of $\dyexact$, $\dsexact$ and $\dxexact$ given in eqn.~(\ref{eq:normal_exact}). Thus,
%
\begin{flalign*}
    \Db^{-1}\dxexact - \Db\dsexact 
    &= \Db^{-1}(-\xb + \sigma \mu \Sb^{-1}\one_n - \Db^2 \dsexact) - \Db\dsexact 
    \\&= \Db^{-1}(-\xb+\sigma\mu \Sb^{-1}\one_n) - 2\Db\dsexact \\
    %
    &= \Db^{-1}(-\xb+\sigma\mu \Sb^{-1}\one_n) - 2(\Ab\Db)^\dagger \Ab (-\xb + \sigma \mu \Sb^{-1}\one_n) \\
    %
    &= (\Db^{-1}-2(\Ab\Db)^\dagger \Ab)(-\xb + \sigma \mu \Sb^{-1}\one_n) \\
    %
    &= (\Db^{-1}-2(\Ab\Db)^\dagger \Ab)\Db\Db^{-1}(-\Xb\one_n + \sigma \mu \Sb^{-1}\one_n) \\
    %
    &= (\Ib-2(\Ab\Db)^\dagger \Ab\Db)[(\Xb\Sb)^{-1/2}(-\Xb\Sb \one_n+\sigma\mu \one_n)].
    %
\end{flalign*}
%
At this point, we have shown that 
\begin{gather}
    \Bcal_2 \leq \|\Ib-2(\Ab\Db)^\dagger \Ab\Db\|_2 \|(\Xb\Sb)^{-1/2}(-\Xb\Sb \one_n+\sigma\mu \one_n)\|_2 \|(\Ab\Db)^\dagger \fb\|_2.\label{eq:pcu_intermediate_b2}
\end{gather}
%    
We can now use the fact that the two-norm of $\Ib-2(\Ab\Db)^\dagger \Ab\Db = \Ib - (\Ab\Db)^\dagger \Ab\Db - (\Ab\Db)^\dagger \Ab\Db$ is upper bounded by two, since $\Ib - (\Ab\Db)^\dagger \Ab\Db$ and $(\Ab\Db)^\dagger \Ab\Db$ are both projection matrices and have two-norm at most one. Next, we bound the middle term, namely $\|(\Xb\Sb)^{-1/2}(-\Xb\Sb e+\sigma\mu \one_n)\|_2$; the proof will use the fact that $(\xb, \yb, \sbb) \in \Ncal_2(\theta)$, which implies that $\|\xb \circ \sbb - \mu\one_n\|_2 \leq \theta \mu$:
%
\begin{flalign*}
    \|(\Xb\Sb)^{-1/2}(-\Xb\Sb\one_n+\sigma\mu \one_n)\|_2^2 
    &= \sum_{i=1}^n \frac{(-\xb_i \sbb_i + \sigma \mu)^2}{\xb_i \sbb_i}
    \leq \frac{\|\xb \circ \sbb - \sigma\mu \one_n\|_2^2}{\min_i \xb_i \sbb_i} \\
    &\leq \frac{\|\xb \circ \sbb - \sigma\mu \one_n\|_2^2}{(1-\theta)\mu}
    \leq \frac{\|(\xb\circ \sbb - \mu \one_n) + (1-\sigma)\mu \one_n\|_2^2}{(1-\theta)\mu} \\
    &\leq \frac{[(\xb\circ \sbb - \mu \one_n) + (1-\sigma)\mu \one_n]^T[(\xb\circ \sbb - \mu \one_n) + (1-\sigma)\mu \one_n]}{(1-\theta)\mu} \\
    &\leq \frac{\|\xb\circ \sbb - \mu \one_n\|_2^2 + 2(1-\sigma)\mu \one_n^T (\xb\circ \sbb - \mu \one_n) + (1-\sigma)^2 \mu^2 n}{(1-\theta)\mu} \\
    &\leq \frac{\|\xb\circ \sbb - \mu \one_n\|_2^2 + 2(1-\sigma)\mu (n\mu - n\mu) + (1-\sigma)^2 \mu^2 n}{(1-\theta)\mu} \\
    &\leq \frac{\theta^2\mu^2 + (1-\sigma)^2\mu^2n}{(1-\theta)\mu} 
    \leq \frac{(\theta^2 + (1-\sigma)^2n)\mu}{(1-\theta)}.
\end{flalign*}    

Inserting the bounds for $\|\Ib-2(\Ab\Db)^\dagger \Ab\Db\|_2$ and $\|(\Xb\Sb)^{-1/2}(-\Xb\Sb\one_n+\sigma\mu \one_n)\|_2$ into the previous bound for $\Bcal_2$ gives:
%
\begin{gather*}
    \Bcal_2 \leq 2 \sqrt{\frac{(\theta^2 + (1-\sigma)^2n)\mu}{(1-\theta)}} \|(\Ab\Db)^\dagger \fb\|_2.
\end{gather*}

Finally, we bound $\Bcal_3$ using properties of the Hadamard product (see Lemma~\ref{lemma:hadamard_cauchy}):   
\begin{flalign}
    \Bcal_3 &= \|[\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb] \circ [\Db^2\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb ]  \|_2 \nonumber\\
    &= \|[\Db\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb] \circ [\Db\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb ]  \|_2 \nonumber\\
    &= \|\Db\Ab^T(\Ab\Db^2\Ab^T)^{-1}\fb\|_2^2 \nonumber\\
    &= \|(\Ab\Db)^T((\Ab\Db)(\Ab\Db)^T)^{-1} \fb\|_2^2 \nonumber\\
    &= \|(\Ab\Db)^\dagger \fb\|_2^2. 
\end{flalign}

Adding the bounds on $\Bcal_1$, $\Bcal_2$, and $\Bcal_3$ gives the final inequality:
\begin{gather*}
        \|\dxtilde \circ \dstilde\|_2
        \leq \frac{\theta^2+n(1-\sigma)^2}{2^{3/2} (1-\theta)} \mu 
        + 2\sqrt{\frac{(\theta^2+n(1-\sigma)^2) \mu}{(1-\theta)}}  \|(\Ab\Db)^\dagger \fb\|_2
        + \|(\Ab\Db)^\dagger \fb\|_2^2.
    \end{gather*}
    
\end{proof}

The next lemma will bound the value of $\|\xtilde(\alpha) \circ \stilde(\alpha) - \mutilde(\alpha) \one_n\|_2$, which will allow us to later show that the iterates remain in the correct neighborhood for a given step size.

\begin{lemma} \label{lemma:pcu_neighborhood_bound}
If $\alpha \in [0,1]$, then
\begin{equation*}
    \|\xtilde(\alpha) \circ \stilde(\alpha) - \mutilde(\alpha) \one_n\|_2
    \leq (1-\alpha)\|\xb \circ \sbb - \mu \one_n\|_2 + \alpha^2\|\dxtilde \circ \dstilde\|_2 + \alpha^2 \|(\Ab\Db)^\dagger \fb\|_2^2.
\end{equation*}
\end{lemma}

\begin{proof}

First, we derive an expression for the difference in the duality measure between the exact and inexact step, $(\mu(\alpha) - \mutilde(\alpha))$. We begin by expanding the definition of $n(\mu(\alpha) - \mutilde(\alpha))$.
\begin{flalign*}
    n(\mu(\alpha) - \mutilde(\alpha)) &= (\xb+\alpha\dxexact)^T(\sbb+\alpha\dsexact)
    - (\xb+\alpha\Delta \xtilde)^T(\sbb+\alpha\Delta \stilde) \nonumber\\
    %
    &= (\xb^T\sbb + \alpha\dxexact^T\sbb + \xb^T \alpha\dsexact + \alpha^2\dxexact^T \dsexact)
    - (\xb^T\sbb + \alpha\Delta \xtilde^T\sbb + \xb^T \alpha\Delta \stilde + \alpha^2\Delta \xtilde^T \Delta \stilde) \nonumber \\
    %
    &= \alpha(\dxexact - \Delta \xtilde)^T\sbb + \alpha \xb^T(\dsexact - \Delta \stilde) + \alpha^2(\dxexact - \Delta \xtilde)^T(\dsexact - \Delta \stilde) \nonumber\\
    %
\end{flalign*}

We next substitute the differences between the exact and inexact steps given by eqns. (\ref{eq:ls_s_diff}, \ref{eq:ls_x_diff}).  We do this in two parts for clearer exposition.
\begin{flalign*}
     \alpha(\dxexact - \Delta \xtilde)^Ts + \alpha \xb^T(\dsexact - \Delta \stilde)
     &= \alpha[\Db^2\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb]^T\sbb + \alpha \xb^T[-\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb] \\
     &= \alpha \fb^T (\Ab\Db^2\Ab^T)^{-1} \Ab \Db^2\sbb
     - \alpha \xb^T\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb \\
     &= \alpha \fb^T (\Ab\Db^2\Ab^T)^{-1} \Ab \Xb\Sb^{-1}\sbb
     - \alpha \xb^T\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb \\
     &= \alpha \fb^T (\Ab\Db^2\Ab^T)^{-1} \Ab \xb
     - \alpha \xb^T\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb \\
     &= 0.
\end{flalign*}

Therefore, substituting this result into the previous set of equations, we get the following.
\begin{flalign}
    n(\mu(\alpha) - \mutilde(\alpha)) 
    &= \alpha^2(\dxexact - \Delta \xtilde)^T(\dsexact - \Delta \stilde) \nonumber\\
    &= \alpha^2[\Db^2\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb]^T [-\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb] \nonumber\\
    &= -\alpha^2 \fb^T (\Ab\Db^2\Ab^T)^{-1}(\Ab\Db^2\Ab^T) (\Ab\Db^2\Ab^T)^{-1} \fb \nonumber \\
    &= -\alpha^2 \fb^T (\Ab\Db^2\Ab^T)^{-1} \fb \Rightarrow \nonumber\\
    \mu(\alpha) - \mutilde(\alpha) &= \frac{-\alpha^2}{n}\|(\Ab\Db)^\dagger \fb\|_2^2, \label{eq:pcu_mu_diff}
\end{flalign}
where the final line follows from properties of the pseudoinverse.
% 
Next, we prove two identities that will be useful.  For the first identity, we expand the term $\xb_i(\alpha)\sbb_i(\alpha)$ and insert eqn.~(\ref{eq:exact_mu_alpha_bound}) to cancel terms:
%
\begin{align}
    \xb_i(\alpha)\sbb_i(\alpha) - \mu(\alpha)
    &= \xb_i \sbb_i + \alpha(\xb_i\dsexact_i + \dxexact_i \sbb_i) + \alpha^2\dxexact_i \dsexact_i - (1-\alpha(1-\sigma))\mu \nonumber\\
    &= (1-\alpha)\xb_i \sbb_i + \alpha \sigma \mu + \alpha^2\dxexact_i \dsexact_i - (1-\alpha+ \alpha\sigma)\mu \nonumber\\
    &=(1-\alpha)(\xb_i \sbb_i - \mu) + \alpha^2 \dxexact_i \dsexact_i.
\end{align}
%
For the second identity, we expand terms and substitute eqns.~(\ref{eq:ls_s_diff}) and~(\ref{eq:ls_x_diff}) for $\dsexact - \dstilde$ and $\dxexact - \dxtilde$, respectively:
%
\begin{align}
    &\xb_i(\alpha) \sbb_i(\alpha) - \xtilde(\alpha)_i  \stilde(\alpha)_i\nonumber\\
    &= \xb_i\sbb_i + \alpha(\xb_i\dsexact_i + \dxexact_i s_i) + \alpha^2 \dxexact_i \dsexact_i - [\xb_i\sbb_i + \alpha(\xb_i\dstilde_i + \dxtilde_i \sbb_i) + \alpha^2 \dxtilde_i \dstilde_i] \nonumber\\
    &=\alpha[\xb_i(\dsexact_i-\dstilde_i) + \sbb_i(\dxexact_i-\dxtilde_i)] + \alpha^2(\dxexact_i \dsexact_i - \dxtilde_i \dstilde_i)  \nonumber \\
    &= \alpha[\xb\circ (-\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb) + \sbb\circ( \Db^2\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb)]_i + \alpha^2(\dxexact_i \dsexact_i - \dxtilde_i \dstilde_i) \nonumber \\
    &= \alpha[\xb\circ (-\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb) + \xb\circ(\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb)]_i + \alpha^2(\dxexact_i \dsexact_i - \dxtilde_i \dstilde_i) \nonumber \\
    &= \alpha^2(\dxexact_i \dsexact_i - \dxtilde_i \dstilde_i).
\end{align}
%
using the above two identities, we expand and rearrange $\xtilde(\alpha)_i\stilde(\alpha)_i - \mutilde(\alpha)$ to get:
%
\begin{align*}
    \xtilde(\alpha)_i\stilde(\alpha)_i - \mutilde(\alpha)
    &= \xb(\alpha)_i \sbb(\alpha)_i - (\xb(\alpha)_i \sbb(\alpha)_i - \xtilde(\alpha)_i  \stilde(\alpha)_i) - [\mu(\alpha) - (\mu(\alpha) - \mutilde(\alpha))] \\
    %
    &= [\xb(\alpha)_i \sbb(\alpha)_i - \mu(\alpha) ] - (\xb(\alpha)_i \sbb(\alpha)_i - \xtilde(\alpha)_i  \stilde(\alpha)_i) + (\mu(\alpha) - \mutilde(\alpha)) \\
    %
    &= [(1-\alpha)(\xb_i \sbb_i - \mu) + \alpha^2 \dxexact_i \dsexact_i] - (\xb(\alpha)_i \sbb(\alpha)_i - \xtilde(\alpha)_i  \stilde(\alpha)_i) + (\mu(\alpha) - \mutilde(\alpha)) \\
    %
    &=  (1-\alpha)(\xb_i \sbb_i - \mu) + \alpha^2 \dxexact_i \dsexact_i - \alpha^2(\dxexact_i \dsexact_i - \dxtilde_i \dstilde_i) + (\mu(\alpha) - \mutilde(\alpha)) \\
    %
    &= (1-\alpha)(\xb_i \sbb_i - \mu) + \alpha^2\dxtilde_i \dstilde_i + (\mu(\alpha) - \mutilde(\alpha)).
\end{align*}
%
Taking vector norms of the above element-wise equality and substituting eqn.~(\ref{eq:pcu_mu_diff}) for $\mu(\alpha) - \mutilde(\alpha)$, we conclude,
%
\begin{align*}
    \|\xtilde(\alpha) \circ \stilde(\alpha) - \mutilde(\alpha) \one_n\|_2
    &\leq (1-\alpha)\|\xb \circ \sbb - \mu \one_n\|_2 + \alpha^2\|\dxtilde \circ \dstilde\|_2 + \|(\mu(\alpha) - \mutilde(\alpha))\one_n\|_2 \\
    %
    &\leq (1-\alpha)\|\xb \circ \sbb - \mu \one_n\|_2 + \alpha^2\|\dxtilde \circ \dstilde\|_2 + \alpha^2 \|(\Ab\Db)^\dagger \fb\|_2^2.
\end{align*}
\end{proof}

Next, we prove that the predictor stays in the slightly enlarged neighborhood $\Ncal_2(0.5)$ when starting from the smaller neighborhood $\Ncal_2(0.25)$.  We will later show that the corrector step guarantees that the iterate ``returns'' to the ``correct'' $\Ncal_2(0.25)$ neighborhood.  Recall that $\sigma = 0$ in the predictor step to get the following lemma.
%
\begin{lemma}\label{lemma:pcu_predictor_step_size}
    If $(\xb,\yb,\sbb) \in \Ncal_2(0.25)$,
\begin{equation*}
    \alpha = \min \left\{
    1/2,  \left( \frac{\mu}{16(\|\dxtilde \circ \dstilde\|_2)} \right)^{1/2}
    \right\},
    ~~~~~
    \|(\Ab\Db)^\dagger \fb\|_2 \leq \frac{\sqrt{\mu}}{2},
\end{equation*} 
    then the predictor step $(\xtilde(\alpha), \ytilde(\alpha), \stilde(\alpha)) \in \Ncal_2(0.5)$.
\end{lemma}

\begin{proof}
We begin with the inequality of Lemma~\ref{lemma:pcu_neighborhood_bound}.  Recall that $\|\xb \circ \sbb - \mu \one_n\|_2 \leq \nicefrac{\mu}{4}$ since $(\xb, \yb, \sbb) \in \Ncal(0.25)$:
%
\begin{align*}
    \|\xtilde(\alpha) \circ \stilde(\alpha) - \mutilde(\alpha) \one_n\|_2
    &\leq (1-\alpha)\|\xb \circ \sbb - \mu \one_n\|_2 + \alpha^2\|\dxtilde \circ \dstilde\|_2 + \alpha^2\|(\Ab\Db)^\dagger \fb\|_2^2 \\
    %
    &\leq (1-\alpha)\|\xb \circ \sbb - \mu \one_n\|_2 + \frac{\mu(\|\dxtilde \circ \dstilde\|_2)}{16(\|\dxtilde \circ \dstilde\|_2} + \frac{1}{2^2} \frac{\mu}{4}\\
    %
    &\leq \frac{(1-\alpha)\mu}{4} + \frac{1}{8(1-\alpha)} (1-\alpha)\mu
    ~~~~(\text{since }(\xb,\yb,\sbb) \in \Ncal_2(0.25)) \\
    %
    &\leq \frac{(1-\alpha)\mu}{4} + \frac{(1-\alpha)\mu}{4}
    ~~~~(\text{since } \alpha \leq \nicefrac{1}{2}) \\
    %
    &\leq \frac{1}{2} (1-\alpha)\mu \leq \frac{1}{2}\mutilde(\alpha).
%
\end{align*}
%
The last line follows from eqn.~(\ref{eq:exact_mu_alpha_bound}), which gives $\mu(\alpha) = (1-\alpha)\mu$ for $\sigma=0$.  We also know from eqn.~(\ref{eq:pcu_mu_diff}) that $\mutilde(\alpha) \geq \mu(\alpha)$. Therefore, $\|\xtilde(\alpha) \circ \stilde(\alpha) - \mutilde(\alpha) \one_n\|_2 \leq \nicefrac{1}{2}\,\mutilde(\alpha)$. Now, we must show that the condition $(\xtilde(\alpha), \stilde(\alpha)) > 0$ is fulfilled. First, by eqns. (\ref{eq:exact_mu_alpha_bound}, \ref{eq:pcu_mu_diff}), we have $\mutilde(\alpha) = [1 - \alpha(1-\sigma)]\mu + \frac{\alpha^2}{n}\|(\Ab\Db)^\dagger \fb\|_2^2$, which shows $\mutilde(\alpha') > 0$ for all positive step sizes $\alpha' \leq \alpha$.  From the first part of this proof, we have that $\xtilde_i(\alpha)\stilde_i(\alpha) \geq \nicefrac{1}{2} \mutilde(\alpha)$. We conclude that $(\xtilde(\alpha), \ytilde(\alpha), \stilde(\alpha)) \in \Ncal_2(0.5)$.

\end{proof}

The next lemma shows that the step size given in the previous lemma will result in a multiplicative decrease in the duality gap during the predictor step.

\begin{lemma} \label{lemma:pcu_predictor_step}
If $(\xb,\yb,\sbb) \in \Ncal_2(0.25)$,
\begin{equation*}
        \alpha = \min \left\{
        1/2,  \left( \frac{\mu}{16(\|\dxtilde \circ \dstilde\|_2)} \right)^{1/2}
        \right\},
        ~~~~\text{and}~~~~
        \|(\Ab\Db)^\dagger \fb\|_2 \leq \frac{\sqrt{\mu}}{8},
\end{equation*}
then the predictor step $(\xtilde(\alpha), \ytilde(\alpha), \stilde(\alpha)) \in \Ncal_2(0.5)$ and there exists a constant $C_0 \in (0,1)$ such that,
%
\begin{equation*}
    \frac{\mutilde(\alpha)}{\mu} \leq 1 - \frac{C_0}{\sqrt{n}}.
\end{equation*}
%
\end{lemma}
%
We note that in the above lemma $(\xtilde(\alpha), \ytilde(\alpha), \stilde(\alpha))$ is the output after the predictor step \textit{only}, before the corrector step is applied.
%
\begin{proof}

To lower bound the decrease in the duality gap at each step, we first find a lower bound for the step size $\alpha$, using the upper bound for $\|\dxtilde \circ \dstilde\|_2$.  By Lemma \ref{lemma:pcu_cross_bound}, we have the following inequality:
\begin{gather*}
    \|\dxtilde \circ \dstilde\|_2
    \leq \frac{\theta^2+n(1-\sigma)^2}{2^{3/2} (1-\theta)} \mu 
    + 2\sqrt{\frac{(\theta^2+n(1-\sigma)^2) \mu}{(1-\theta)}}  \|(\Ab\Db)^\dagger \fb\|_2
    + \|(\Ab\Db)^\dagger \fb\|_2^2.
\end{gather*}

We can simplify this inequality by substituting $\|(\Ab\Db)^\dagger \fb\|_2 \leq \sqrt{\mu}/8$, $\theta = 0.25$, and $\sigma=0$ to get:
%
\begin{flalign*}
    \|\dxtilde \circ \dstilde\|_2
    &\leq \frac{(0.25)^2+n(1-0)^2}{2^{3/2} (1-0.25)} \mu 
    + 2\sqrt{\frac{(0.25^2+n(1-0)^2) \mu}{(1-0.25)}} \frac{\sqrt{\mu}}{8}
    + \frac{\mu}{64} \\
    &\leq \frac{1/16+n}{2^{3/2} (3/4)} \mu 
    + 2\sqrt{\frac{(1/16+n) \mu}{3/4}} \frac{\sqrt{\mu}}{8}
    + \frac{\mu}{64} \\
    &\leq n\mu\left(\frac{1/16+1}{2^{3/2} (3/4)} 
    + 2\sqrt{\frac{(1/16+1)}{3/4}} \frac{1}{8}
    + \frac{1}{64}\right) \\
    &\leq 0.82\cdot n\mu.
\end{flalign*}
%
We can now insert the upper bounds for $\|\dxtilde \circ \dstilde\|_2$ and $\|(\Ab\Db)^\dagger \fb\|_2$ to lower bound $\alpha$:
%
\begin{flalign*}
    \alpha 
    &= \min \left\{1/2,  \left( \frac{\mu}{8(\|\dxtilde \circ \dstilde\|_2 + \|(\Ab\Db)^\dagger \fb\|_2^2)} \right)^{1/2}
    \right\} \\
    &\geq \min \left\{1/2,  \left( \frac{\mu}{8 (0.82) n \mu + \mu/8} \right)^{1/2}
    \right\} \\
    &\geq \min \left\{1/2,  \left( \frac{1}{n(6.56 + 1/8)} \right)^{1/2}
    \right\} \\
    &\geq \sqrt{\nicefrac{0.14}{n}}.
\end{flalign*}
%
We proceed by using eqns.~(\ref{eq:exact_mu_alpha_bound}) and (\ref{eq:pcu_mu_diff}) to upper bound $\mutilde(\alpha)$. We substitute the upper bound for $\|(\Ab\Db)^\dagger \fb\|_2$ as well as the upper and lower bounds for $\alpha$ as needed to derive a worst case bound. Recall that the step size $\alpha$ is upper bounded by $1/2$ (by definition):
%
\begin{flalign*}
    \mutilde(\alpha) 
    &\leq \mu(\alpha) - [\mu(\alpha) - \mutilde(\alpha)] 
    \leq (1-\alpha)\mu + \frac{\alpha^2}{n}\|(\Ab\Db)^\dagger \fb\|_2^2 \\
    &\leq \left(1-\alpha\right)\mu + \frac{\alpha^2\mu}{64n} 
    \leq \left(1-\sqrt{\frac{0.14}{n}}\right)\mu + \frac{\mu}{4\cdot64n} \\
    &\leq \left[\left(1-\sqrt{\frac{0.14}{n}}\right) + \frac{1}{4\cdot64\sqrt{n}}\right]\mu
    \leq \left[1 - \frac{\sqrt{0.14} - (1/256)}{\sqrt{n}}\right]\mu.
\end{flalign*}
%
Then, if we let $C_0 = \sqrt{0.14} - (1/256)$, we get
\begin{gather*}
    \frac{\mutilde(\alpha)}{\mu} \leq 1 - \frac{C_0}{\sqrt{n}},
    ~~~~\text{with }C_0 \in (0,1).
\end{gather*}
%
\end{proof}

So far, We have shown that the predictor step results in a multiplicative decrease in the duality gap while keeping the next iterate in the neighborhood $\Ncal_2(0.5)$.  We now show that the corrector step returns the iterate to the $\Ncal_2(0.25)$ neighborhood while increasing the duality gap by only a small additive amount. 

\begin{lemma} \label{lemma:pcu_corrector_step}
Let $(\xb, \yb, \sbb) \in \Ncal_2(0.5)$ and
$\|(\Ab\Db)^\dagger \fb\|_2 \leq \nicefrac{\sqrt{\mu}}{2^6}$. Then,
the corrector step $(\xtilde(1), \ytilde(1), \stilde(1)) \in \Ncal_2(0.25)$ and $|\mutilde(1) - \mu| \leq \nicefrac{\|(\Ab\Db)^\dagger \fb\|_2^2}{n}$.
\end{lemma}

\begin{proof}
First, we show that taking a step with step size $\alpha = 1$ and centering parameter $\sigma =1$ from a point in $\Ncal_2(0.5)$ ``returns'' that point to the smaller neighborhood $\Ncal_2(0.25)$. We start with the inequality given by Lemma~\ref{lemma:pcu_neighborhood_bound} with $\alpha = 1$ and then substitute the bound for $\|\dxtilde \circ \dstilde\|_2$ from Lemma~\ref{lemma:pcu_cross_bound} to get:
%
\begin{align*}
    \|\xtilde(1) \circ \stilde(1) - \mutilde(1)\|_2
    &\leq \|\dxtilde \circ \dstilde\|_2 + \|(\Ab\Db)^\dagger \fb\|_2^2 \\
    %
    &\leq 
    \frac{\theta^2+n(1-\sigma)^2}{2^{3/2} (1-\theta)} \mu 
    + 2\sqrt{\frac{(\theta^2+n(1-\sigma)^2) \mu}{(1-\theta)}}  \|(\Ab\Db)^\dagger \fb\|_2
    + 2\|(\Ab\Db)^\dagger \fb\|_2^2.
\end{align*}
%
Next, we use $\|(\Ab\Db)^\dagger \fb\|_2 \leq \sqrt{\mu}/2^6$, $\theta = 0.5$, and $\sigma = 1$:
%
\begin{flalign*}
    \|\xtilde(1) \circ \stilde(1) - \mutilde(1)\|_2
    &\leq \frac{(0.5)^2+n(1-1)^2}{2^{3/2} (1-0.5)} \mu 
    + 2\sqrt{\frac{((0.5)^2+n(1-1)^2) \mu}{(1-0.5)}}  \frac{\sqrt{\mu}}{2^6}
    + \frac{2\mu}{2^{12}} \\
    &\leq \frac{(1/4)}{2^{3/2} (1/2)} \mu 
    + 2\sqrt{\frac{(1/4) \mu}{(1/2)}}  \frac{\sqrt{\mu}}{2^6}
    + \frac{2\mu}{2^{12}} \\
    &\leq \frac{\mu}{2^{9/2}} + \frac{\mu}{2^{11/2}} + \frac{\mu}{2^{11}} \leq \frac{1}{4} \mu.
\end{flalign*}

Again, $\mutilde(\alpha) \geq \mu(\alpha)$ which implies that $\|\xtilde(1) \circ \stilde(1) - \mutilde(1)\|_2 \leq \nicefrac{1}{4}\,\mutilde(1)$, so we can conclude that $(\xtilde(1), \ytilde(1), \stilde(1)) \in \Ncal_2(0.25)$.

Finally, we show that the duality gap increases only slightly.  In the exact case, the duality gap does not increase at all when $\sigma = 1$, i.e. $\mu(1) = \mu$, as can be seen in eqn.~(\ref{eq:exact_mu_alpha_bound}). Therefore, by looking at the difference between the exact and inexact duality gaps, i.e. eqn.~(\ref{eq:pcu_mu_diff}), we get
%
\begin{gather*}
    |\mutilde(1)-\mu(1)| \leq  \frac{\|(\Ab\Db)^\dagger \fb\|_2^2}{n} 
    \Rightarrow |\mutilde(1)-\mu| \leq \frac{\|(\Ab\Db)^\dagger \fb\|_2^2}{n}.
\end{gather*}
%
\end{proof}
%

Finally, we combine the results of the previous lemmas with a standard convergence argument to show the overall correctness and convergence rate of Algorithm~\ref{algo:pcu}, namely the \textit{inexact} Predictor-Corrector IPM, thus proving Theorem~\ref{thm:pcu_final}. 

\begin{proof}(of Theorem \ref{thm:pcu_final})
%
We introduce the following notation to more easily discuss the steps of Algorithm \ref{algo:pcu}.  Let $(\dxtilde_p, \dytilde_p, \dstilde_p)$ denote the predictor step computed by steps (a-b) and $(\dxtilde_c, \dytilde_c, \dstilde_c)$ denote the corrector step computed by steps (e-f). 

Algorithm~\ref{algo:pcu} first computes the predictor step from $\dytilde_p = \solve(\Ab\Db^2\Ab^T, \Ab\xb, \tolSolve)$ and then computes the corrector step from $\dytilde_c = \solve(\Ab\Db^2\Ab^T, -\mu\Ab\Sb^{-1}\one_n + \Ab\xb, \tolSolve)$.  Let $\fb_p$ and $\fb_c$ denote the error vectors incurred when solving for the predictor and corrector steps, respectively. Guarantee (i) of $\solve$ (see eqn.~(\ref{eq:solve_def})) allows us to bound the term $\|(\Ab\Db)^\dagger \fb\|_2$ as follows: 
%
\begin{gather}
    \|\dytilde-(\Ab\Db^2\Ab^T)^{-1}(-\sigma \mu \Ab\Sb^{-1}\one_n + \Ab\xb)\|_{\Ab\Db^2\Ab^T} \leq \tolSolve \nonumber\\
    %
    \Rightarrow \|\dytilde-\dyexact\|_{\Ab\Db^2\Ab^T} \leq \tolSolve \nonumber\\
    %
    \Rightarrow \|\dytilde-\dyexact\|_{\Ab\Db^2\Ab^T} \leq \tolSolve \nonumber\\
    %
    \Rightarrow \|(\Ab\Db^2\Ab^T)^{-1} \fb\|_{\Ab\Db^2\Ab^T} \leq \tolSolve \nonumber\\
    %
    \Rightarrow \|(\Ab\Db)^\dagger \fb\|_2 \leq \tolSolve. \label{eq:solve1_bound}
\end{gather}
%
Thus, we have the following bounds, using the value of $\tolSolve$ in Theorem \ref{thm:pcu_final}:
%
\begin{gather*}
    \|(\Ab\Db)^\dagger \fb_p\|_2,
    ~
    \|(\Ab\Db)^\dagger \fb_c\|_2 \leq \nicefrac{\sqrt{\epsilon}}{2^6}.
\end{gather*}
%
Algorithm~\ref{algo:pcu} sets the step size $\alpha$ for the predictor step to the value given by Lemma~\ref{lemma:pcu_predictor_step_size}.  If $(\xb_0, \yb_0, \sbb_0) \in \Ncal_2(0.25)$ and $\mu_0 \geq 2\epsilon$, then Lemma~\ref{lemma:pcu_predictor_step} guarantees that the predictor step will reduce the duality gap by a multiplicative factor of $1 - \nicefrac{C_0}{\sqrt{n}}$, while keeping the iterate in the neighborhood $\Ncal_2(0.5)$. Lemma~\ref{lemma:pcu_corrector_step} then guarantees that the ensuing corrector step will return the iterate to the neighborhood $\Ncal_2(0.25)$, while increasing the duality measure by at most $\nicefrac{\tolSolve}{n}$.  Therefore, a single iteration of Algorithm~\ref{algo:pcu}, starting from a point $(\xb_0, \yb_0, \sbb_0) \in \Ncal_2(0.25)$ such that $\mu_0 \geq 2\epsilon$ guarantees:
%
\begin{gather*}
    \mu_1 \leq \left(1 - \frac{C_0}{\sqrt{n}}\right)\mu_0 +  \frac{\epsilon C_0}{2 \sqrt{n} \log \mu_0/\epsilon}.
\end{gather*}

This fulfills the conditions of Lemma \ref{lemma:ipm_convergence} with $C_0 \in (0,1)$ and $C_1 \leq \frac{C_0}{2 \sqrt{n} \log \mu_0/\epsilon} \leq \nicefrac{C_0}{\sqrt{n}}$. Therefore, we conclude that Algorithm~\ref{algo:pcu} converges after $\frac{\sqrt{n}}{C_0} \log \frac{\mu_0}{\epsilon}$ outer iterations iterations.

We now prove that the final iterate of Algorithm~\ref{algo:pcu}, which we denote by $(\xtopt, \ytopt, \stopt)$, is $\epsilon$-feasible. In a single iteration, the primal variable changes by $\dxtilde = \dxtilde_p + \dxtilde_c$. Let $\fb = \fb_p + \fb_c$ and recall that by the second guarantee of $\solve$, $\|\Ab\Db^2\Ab^T \dytilde - \pb \|_2 \leq \tolSolve$.  This is equivalent to $\|\fb_p\|_2, \|\fb_c\|_2 \leq \tolSolve$ for all iterations of Algorithm~\ref{algo:pcu}. We proceed by showing that the change in the primal residual at the $k$-th iteration is exactly $\fb_k$: 
%
\begin{flalign*}
    \|\Ab\xb_k - \Ab\xb_{k-1}\|_2 
    &= \|\Ab(\xb_{k-1} + \dxtilde_{k-1}) - \Ab\xb_{k-1}\|_2
    = \|\Ab\dxtilde_{k-1}\|_2 \\
    &= \|\Ab(\dxexact_{k-1} - \dxtilde_{k-1})\|_2 
    =  \|\Ab(\Db^2\Ab^T(\Ab\Db^2\Ab^T)^{-1} \fb_{k-1})\|_2
    = \|\fb_{k-1}\|_2.
\end{flalign*}

We can use the bound $\|\fb_i\|_2 \leq 2\tolSolve$ to bound the primal residual at the $k$-th iteration.
\begin{flalign*}
    \|\bb - \Ab\xb_k\|_2
    &= \|\bb - \Ab\xb_1 + (\Ab\xb_2 - \Ab\xb_1) + ... + (\Ab\xb_k - \Ab\xb_{k-1})\|_2\\
    &= \|(\Ab\xb_0 - \Ab\xb_1) + (\Ab\xb_2 - \Ab\xb_1) +  ... + (\Ab\xb_k - \Ab\xb_{k-1})\|_2\\
    &\leq \|\Ab\xb_0 - \Ab\xb_1\|_2 + \|\Ab\xb_2 - \Ab\xb_1\| + ... + \|\Ab\xb_k - \Ab\xb_{k-1}\|_2 \\
    &\leq \|\fb_0\|_2 + \|\fb_1\|_2 + ... + \|\fb_{k-1}\|_2
    \leq 2k\tolSolve.
\end{flalign*}

We previously concluded in this proof by Lemma \ref{lemma:ipm_convergence} that the Algorithm \ref{algo:pcu} will converge after $k = \frac{\sqrt{n}}{C_0} \log \frac{\mu_0}{\epsilon}$ iterations.  By the conditions of Theorem \ref{thm:pcu_final}, $\tolSolve < \frac{\epsilon C_0}{2 \sqrt{n} \log \mu_0/\epsilon}$.  Therefore, we conclude that $\|\Ab\xtopt - \bb\|_2 \leq \epsilon$, i.e. the solution is $\epsilon$-primal feasible. 

%
\end{proof}






